Boosting Adversarial Training via Fisher-Rao Norm-based Regularization

Adversarial training is extensively utilized to improve the adversarial robustness of deep neural networks. Yet, mitigating the degradation of standard generalization performance in adversarial-trained models remains an open problem. This paper attempts to resolve this issue through the lens of model complexity. First, We leverage the Fisher-Rao norm, a geometrically invariant metric for model complexity, to establish the non-trivial bounds of the Cross-Entropy Loss-based Rademacher complexity for a ReLU-activated Multi-Layer Perceptron. Then we generalize a complexity-related variable, which is sensitive to the changes in model width and the trade-off factors in adversarial training. Moreover, intensive empirical evidence validates that this variable highly correlates with the generalization gap of Cross-Entropy loss between adversarial-trained and standard-trained models, especially during the initial and final phases of the training process. Building upon this observation, we propose a novel regularization framework, called Logit-Oriented Adversarial Training (LOAT), which can mitigate the trade-off between robustness and accuracy while imposing only a negligible increase in computational overhead. Our extensive experiments demonstrate that the proposed regularization strategy can boost the performance of the prevalent adversarial training algorithms, including PGD-AT, TRADES, TRADES (LSE), MART, and DM-AT, across various network architectures. Our code will be available at https://github.com/TrustAI/LOAT.

==> Tabs/Generalization_Gap.tex <==
\begin{table}[htbp]
\scriptsize
\setlength{\tabcolsep}{3pt}
\centering
\begin{tabular}{c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{Defense}& \multicolumn{3}{c|}{ResNet18} & \multicolumn{3}{c}{WRN-34-10} \\
& {\tiny$\tilde{R}_{N_1}(\mathcal{L}_{ce})$} & {\tiny$\tilde{R}_{N_2}(\mathcal{L}_{ce})$} & Diff. & {\tiny$\tilde{R}_{N_1}(\mathcal{L}_{ce})$} & {\tiny$\tilde{R}_{N_2}(\mathcal{L}_{ce})$} & Diff. \\
\hline
MART & Data & Data & Data
& Data & Data & Data \\
MART\textcolor{red}{*}$^{\dag}$ & Data & Data & Data
& Data & Data & Data \\
\hline
TRADES & 0.5343 & 0.7345 & 0.2002
& Data & Data & Data \\
TRADES\textcolor{red}{*}$^{\dag}$ & 0.5343 & 0.7345 & 0.2002
& Data & Data & Data \\
\hline
\end{tabular}
\caption{CE loss-based generalization gap on clean images. VGG-13 and VGG-19 are used for evaluations.}
\label{generalization}
\end{table}



==> Tabs/traditional_AT_new.tex <==
\begin{table}[htbp]
\scriptsize
\setlength{\tabcolsep}{4pt}
\centering
\begin{tabular}{c|c|c|c|c|c|c}
\toprule
Models & Defense & Clean$_{tr}$ & Clean$_{te}$ & FGSM & PGD$^{7}$ & PGD$^{20}$ \\
\midrule
\multirow{9}{*}{ResNet18}   & TRADES & 93.39 & 82.23 & 57.89  & \textcolor{blue}{\textbf{53.68}}  & \textcolor{red}{\textbf{52.00}}\\
                            & TRADES\textcolor{red}{*} & \textcolor{blue}{\textbf{94.77}}&\textcolor{blue}{\textbf{82.29}} & \textcolor{blue}{\textbf{62.19}} & 53.32 & 49.77 \\
                            &TRADES\textcolor{red}{*}$^{\dag}$& \textbf{\textcolor{red}{95.35}} &  \textbf{\textcolor{red}{82.51}} &\textbf{\textcolor{red}{62.47}} & \textbf{\textcolor{red}{53.96}} & \textcolor{blue}{\textbf{50.43}}  \\
                            \cmidrule(lr){2-7}
                             & TRADES(S) & \textcolor{blue}{\textbf{92.92}} & 82.95& 58.14 & 54.01 & 52.71 \\
                             & TRADES(S)\textcolor{red}{*} & \textcolor{red}{\textbf{93.25}} & 83.01 & 62.32 & 54.99 & 51.96 \\
                         & TRADES(S)\textcolor{red}{*}$^\dag$ & 92.79 & 82.73 & \textcolor{red}{\textbf{62.76}} & \textcolor{red}{\textbf{54.06}} & \textcolor{red}{\textbf{51.03}} \\    \cmidrule(lr){2-7}
                             & MART & 87.85 & 80.61 & 62.41 & 54.86 & 51.65 \\
                             & MART\textcolor{red}{*} & 90.04 & \textcolor{blue}{\textbf{82.34}} & 59.10 &54.44& \textcolor{red}{\textbf{52.50}} \\
                             & MART\textcolor{red}{*}$^{\dag}$ & 88.26 & 80.41 & \textcolor{blue}{\textbf{62.79}} &\textcolor{blue}{\textbf{54.93}}& 51.22 \\
                             & MART\textcolor{blue}{*} & \textcolor{red}{\textbf{90.14}} & \textcolor{red}{\textbf{82.43}} & 59.24 & 54.40 & \textcolor{blue}{\textbf{52.30}} \\
                             & MART\textcolor{blue}{*}$^{\dag}$ & \textcolor{blue}{\textbf{88.83}} & 81.50 & \textcolor{red}{\textbf{63.66}} & \textcolor{red}{\textbf{55.88}} & 52.28 \\
                             \cmidrule(lr){2-7}
                             & PGD-AT & 96.11 & 82.96 & 53.00 & 46.95 &44.38 \\
                             & PGD-AT\textcolor{red}{*} & 97.01& 83.41 & 53.17 & 47.26 &\textbf{44.58} \\
                             & PGD-AT\textcolor{blue}{*} & \textbf{97.18}&\textbf{83.41} & \textbf{53.49} & \textbf{47.28} &44.48\\
\midrule
\multirow{6}{*}{ResNet50}  
                             & TRADES & 93.89  &
                             83.38&  \textcolor{blue}{\textbf{64.53}} & \textcolor{blue}{\textbf{56.23}} & \textcolor{red}{\textbf{52.39}} \\ 
                             & TRADES\textcolor{red}{*} & \textcolor{blue}{\textbf{94.74}} & \textcolor{red}{\textbf{84.07}} & 64.32 &55.78 & 52.15  \\
                             & TRADES\textcolor{red}{*}$^{\dag}$ & \textcolor{red}{\textbf{94.83}} & \textcolor{blue}{\textbf{83.81}} & \textcolor{red}{\textbf{64.69}} &\textcolor{red}{\textbf{56.30}} & \textcolor{blue}{\textbf{52.34}} \\ \cmidrule(lr){2-7}
                        
\midrule
\end{tabular}
\caption{}
\label{tab}
\end{table}
